GroundingGPT:Language Enhanced Multi-modal Grounding Model

Multi-modal large language models have demonstrated impressive performance across various tasks in different modalities. However, existing multi-modal models primarily emphasize capturing global information within each modality while neglecting the importance of perceiving local information across modalities. Consequently, these models lack the ability to effectively understand the fine-grained details of input data, limiting their performance in tasks that require a more nuanced understanding. To address this limitation, there is a compelling need to develop models that enable fine-grained understanding across multiple modalities, thereby enhancing their applicability to a wide range of tasks. In this paper, we propose GroundingGPT, a language enhanced multi-modal grounding model. Beyond capturing global information like other multi-modal models, our proposed model excels at tasks demanding a detailed understanding of local information within the input. It demonstrates precise identification and localization of specific regions in images or moments in videos. To achieve this objective, we design a diversified dataset construction pipeline, resulting in a multi-modal, multi-granularity dataset for model training. The code, dataset, and demo of our model can be found at https: //github.com/lzw-lzw/GroundingGPT.

==> Sections/demonstration.tex <==
In this section, we will evaluate the performance of the GroundingGPT model from two aspects. Firstly, we will assess whether GroundingGPT can effectively understand various modal inputs. In addition to comprehending the overall information of the inputs, GroundingGPT should be able to capture fine-grained details. Additionally, the model should possess the ability to reason based on both the input and intrinsic knowledge. Secondly, we will examine how well the GroundingGPT model accomplishes grounding tasks across different modalities, which distinguishes it from other models. Consequently, we will showcase GroundingGPT's performance in tasks such as image grounding, video grounding, and audio localization.
\subsection{Multi-modality Understanding}
First, we validated GroundingGPT's understanding and reasoning capabilities with multi-modal inputs. As shown in Figure \ref{fig:image demo}, GroundingGPT is able to observe objects of different granularity in the input image, demonstrating its multi-granularity understanding ability. In the lower part of Figure \ref{fig:image demo}, when asked about funny things in the image, GroundingGPT is also capable of effectively identifying unusual aspects, showcasing a certain level of common-sense reasoning ability. 
When provided with video inputs, GroundingGPT is capable of accurately describing the content of the videos. In the first example in Figure \ref{fig:video demo}, GroundingGPT is able to identify the city depicted in the video description based on its knowledge. Moreover, the model demonstrates a strong understanding of the temporal order of events in the video, thanks to the introduction of temporal positional encoding in its architecture, which preserves the temporal information of the video. Similarly, as shown in Figure \ref{fig:audio demo}, when presented with audio clips as inputs, GroundingGPT can generate corresponding descriptions based on the audio output. 

In summary, the GroundingGPT model possesses the ability to understand inputs from various modalities, respond to human instructions, and perform scene reasoning based on its knowledge, showcasing the foundational capabilities of other multi-modal large language models. 


\subsection{Multi-modal Grounding}
In this section, we evaluate the performance of GroundingGPT in multi-modal grounding tasks. As shown in Figure \ref{fig:image grounding demo}, when inputting an image and requesting the model to output object coordinates, GroundingGPT is capable of generating responses while providing the requested coordinates for mentioned objects. Additionally, when we specify a region of interest in the image for questioning, GroundingGPT can reason based on local information and provide correct answers, demonstrating its effectiveness in image grounding task. 
In Figure \ref{fig:video grounding demo}, when asked to generate video summaries, GroundingGPT can summarize events in this video in the correct temporal order. Furthermore, when inquired about a specific event timestamp, GroundingGPT can accurately generate the corresponding time segment, thanks to the incorporation of temporal information in the model's video branch.
When used for audio localization tasks, the GroundingGPT model is capable of determining the location of the audio source in the image based on the content of the audio and the image. It successfully achieves cross-modal grounding by accurately localizing the audio source in the image.

Overall, by training on the multi-modal and multi-granularity dataset we constructed, GroundingGPT demonstrates not only its ability to comprehend multiple modalities but also its effectiveness in various grounding tasks. It showcases its understanding of fine-grained information, validating the effectiveness of the dataset we created.

==> Tables/ablation.tex <==
\begin{table*}[t]
    \centering
    % \renewcommand\arraystretch{1.5}
    \begin{tabular}{ccccccc|ccc}
    \toprule
    \multirow{2}{*}{Row} & \multirow{2}{*}{LLM Size} &  \multirow{2}{*}{Resolution} & \multirow{2}{*}{Adapter} & \multirow{2}{*}{Stage1} & \multirow{2}{*}{Stage2} & \multirow{2}{*}{Stage3} & \multicolumn{3}{c}{RefCOCO} \\
    \cline{8-10}
    & & & & & & & val & testA & testB \\
    \midrule
    1 & 7B & $224\times224$   & Linear & C & F & C+F & 84.68 & 88.88 & 78.94 \\
    2 & 7B & $224\times224$ & Linear & C+F & F & C+F & 82.43 & 86.87 & 75.37 \\
    3 & 7B & $336\times336$ & Linear & C & F & C+F & 86.01 & 90.45 & 80.43 \\  
    4 & 7B & $336\times336$  & MLP    & C & F & C+F & 88.02 & 91.55 & 82.47 \\
    5 & 13B &$336\times336$  & MLP    & C & F & C+F & \textbf{88.26} & \textbf{92.05} & \textbf{82.65} \\
    % \multirow{2}{*}{Models} & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg}\\
    % \cline{2-9}
    %  & val & testA & testB & val & testA & testB & val & test \\
    % \midrule
    % UNITER       & 81.41 & 87.04 & 74.17 & 75.90 & 81.45 & 66.70 & 74.02 & 68.67\\
    % MDETR        & 86.75 & 89.58 & 81.41 & 79.52 & 84.09 & 70.62 & 81.64 & 80.89\\
    % UniTAB       & 86.32 & 88.84 & 80.61 & 78.70 & 83.22 & 69.48 & 79.96 & 79.97\\
    % \midrule
    % KOSMOS-2     & 52.32 & 57.42 & 47.26 & 45.48 & 50.73 & 42.24 & 60.57 & 61.65\\  
    % Shikra       & 87.01 & 90.61 & 80.24 & 81.60 & 87.36 & 72.12 & 82.27 & 82.19\\
    % NExT-Chat*   & 85.5  & 90.0  & 77.9  & 77.2  & 84.5  & 68.0  & 80.1  & 79.8 \\
    % Ferret*      & 87.49 & 91.35 & 82.45 & 80.78 & 87.38 & 73.14 & 83.93 & 84.76\\
    % \midrule
    % % GroundingGPT(224)    & 83.85 & 89.07 & 81.90 & 79.55 & 86.63 & 71.73 & 80.96 & 81.52\\ 
    % % GroundingGPT(336)    & 86.88 & 90.85 & 82.22 & 80.74 & 86.79 & 72.08 & 81.29 & 83.05  \\
    % GroundingGPT & \textbf{88.02} & \textbf{91.55} & \textbf{82.47} & \textbf{81.61} & 87.18 & \textbf{73.18} & 81.60 & 81.99  \\
    % % GroundingGPT-13B     & 88.54 & 92.20 & 82.75 & 82.61 & 88.16 & 74.19 & 82.56 & 83.50 \\        
    \bottomrule
    \end{tabular}
    \caption{Ablation studies of the model architecture, LLM size and training strategy on the REC task. The stages, denoted as stage 1 to stage 3, represent the training data used in each stage. "C" represents coarse-grained data, while "F" represents fine-grained data.}
    \label{tab:ablation}
\end{table*}

% \begin{table*}[t]
%     \centering
%     % \renewcommand\arraystretch{1.5}
%     \begin{tabular}{ccccc|ccc}
%     \toprule
%     \multirow{2}{*}{Row} & \multirow{2}{*}{LLM Size} &  \multirow{2}{*}{Stage1} & \multirow{2}{*}{Stage2} & \multirow{2}{*}{Stage3} & \multicolumn{3}{c}{RefCOCO} \\
%     \cline{6-8}
%     & & & & &  val & testA & testB \\
%     \midrule
%     1 & 7B    & C+F & F & C+F & 88.02 & 91.55 & 82.47 \\
%     2 & 7B    & C & F & C+F & 88.02 & 91.55 & 82.47 \\
%     3 & 13B    & C & F & C+F & \textbf{88.26} & \textbf{92.05} & \textbf{82.65} \\
%     % \multirow{2}{*}{Models} & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg}\\
%     % \cline{2-9}
%     %  & val & testA & testB & val & testA & testB & val & test \\
%     % \midrule
%     % UNITER       & 81.41 & 87.04 & 74.17 & 75.90 & 81.45 & 66.70 & 74.02 & 68.67\\
%     % MDETR        & 86.75 & 89.58 & 81.41 & 79.52 & 84.09 & 70.62 & 81.64 & 80.89\\
%     % UniTAB       & 86.32 & 88.84 & 80.61 & 78.70 & 83.22 & 69.48 & 79.96 & 79.97\\
%     % \midrule
%     % KOSMOS-2     & 52.32 & 57.42 & 47.26 & 45.48 & 50.73 & 42.24 & 60.57 & 61.65\\  
%     % Shikra       & 87.01 & 90.61 & 80.24 & 81.60 & 87.36 & 72.12 & 82.27 & 82.19\\
%     % NExT-Chat*   & 85.5  & 90.0  & 77.9  & 77.2  & 84.5  & 68.0  & 80.1  & 79.8 \\
%     % Ferret*      & 87.49 & 91.35 & 82.45 & 80.78 & 87.38 & 73.14 & 83.93 & 84.76\\
%     % \midrule
%     % % GroundingGPT(224)    & 83.85 & 89.07 & 81.90 & 79.55 & 86.63 & 71.73 & 80.96 & 81.52\\ 
%     % % GroundingGPT(336)    & 86.88 & 90.85 & 82.22 & 80.74 & 86.79 & 72.08 & 81.29 & 83.05  \\
%     % GroundingGPT & \textbf{88.02} & \textbf{91.55} & \textbf{82.47} & \textbf{81.61} & 87.18 & \textbf{73.18} & 81.60 & 81.99  \\
%     % % GroundingGPT-13B     & 88.54 & 92.20 & 82.75 & 82.61 & 88.16 & 74.19 & 82.56 & 83.50 \\        
%     \bottomrule
%     \end{tabular}
%     \caption{Ablation studies of the model architecture, LLM size and training strategy on the REC task. The stages, denoted as stage 1 to stage 3, represent the training data used in each stage. "C" represents coarse-grained data, while "F" represents fine-grained data.}
%     \label{tab:ablation}
% \end{table*}
